PicPersona-TOD : A Dataset for Personalizing Utterance Style in Task-Oriented Dialogue with Image Persona

Task-Oriented Dialogue (TOD) systems are designed to fulfill user requests through natural language interactions, yet existing systems often produce generic, monotonic responses that lack individuality and fail to adapt to users' personal attributes. To address this, we introduce PicPersona-TOD, a novel dataset that incorporates user images as part of the persona, enabling personalized responses tailored to user-specific factors such as age or emotional context. This is facilitated by first impressions, dialogue policy-guided prompting, and the use of external knowledge to reduce hallucinations. Human evaluations confirm that our dataset enhances user experience, with personalized responses contributing to a more engaging interaction. Additionally, we introduce a new NLG model, Pictor, which not only personalizes responses, but also demonstrates robust performance across unseen domains https://github.com/JihyunLee1/PicPersona.

==> tab_demographic.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage[table,xcdraw]{xcolor}
% % Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \begin{table}[]
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{lr|lrlr}
% \hline
% Gender & \multicolumn{1}{l|}{Ratio(\%)} & Country                                               & \multicolumn{1}{l}{Ratio(\%)} &        Country                                               & \multicolumn{1}{l}{Ratio(\%)}                                               \\
% \hline
% Male   & 45.4                       & USA      & 63.36                     & South Korea                  & 1.12                 \\
% Female & 54.6                       & China                         & 6.73                      & Canada                       & 0.73                 \\ \cline{1-2}
% Age    & \multicolumn{1}{l|}{Ratio(\%)} & United Kingdom                & 6.51                      & Spain                        & 0.68                 \\ \cline{1-2}
% 10's   & 17.12                      & Japan                         & 5.77                      & Russia                       & 0.66                 \\
% 20's   & 40.52                      & India                         & 3.67                      & UAE         & 0.54                 \\
% 30's   & 26.08                      & Germany                                               & 2.47                      & Egypt & 0.43                 \\
% 40's   & 11.75                      & Brazil                        & 2.26                      & Argentina                    & 0.41                 \\
% 50's   & 8.37                       & Mexico & 1.63                      & Kazakhstan                   & 0.22                 \\
% 60's   & 6.16                       & Italy                         & 1.56                      & Saudi Arabia                 & 0.13                 \\
%        &                            & France                        & 1.12                      &                                                      & \multicolumn{1}{l}{} 
% \\ \hline
% \end{tabular}
% }
% \caption{Distributions of gender, age, and demographic of Pic-TOD.}
% \label{tab:demographic}
% \end{table}

==> tab_gpt_compare.tex <==

% \begin{table}
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l crrrrrrr}
% \hline
%  & \multirow{2}{*}{All} & \multicolumn{3}{c}{Age} & &\multicolumn{3}{c}{Emotion}  \\
% \cline{3-5}\cline{7-9}
%  && Senior & Adult & Child & & Pos & Neg & Neu  \\
% \hline
%  \makecell[l]{MultiWoZ\\\quad+\small{\citet{joshi2017personalization}}  }&12.67 & 30.77 & 11.46 & 0.00 && 5.50 & 50.00& 29.73 \\
% Tie & 0.67 & 0.00 & 0.00& 3.57 && 0.00& 0.00 & 2.70 \\
% Pic-TOD & \textbf{86.67} & \textbf{69.23} & \textbf{88.54} & \textbf{96.43} && \textbf{94.5} & \textbf{50.0} & \textbf{67.57} \\
% \hline
%  \makecell[l]{MultiWoZ\\\quad+\small{\citet{toad}}  }
% &5.33 &  11.54 & 5.21 & 0.00 &&1.83 & 25.00 & 13.51 \\
% Tie & 2.00 &0.00& 2.08& 3.57&& 1.83& 0.00& 2.70\\
% Pic-TOD & \textbf{92.67} & \textbf{88.46} & \textbf{92.71} & \textbf{96.43} && \textbf{96.33} & \textbf{75.0} & \textbf{83.78} \\
% \hline
% \end{tabular}
% }
% \caption{Winning ratios (\%) comparison of Pic-TOD with other personalization methods, measured by GPT-4.}
% \label{tab:gpt_task2}
% \end{table}

==> tab_model_compare.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t!]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lrrrrrrrr}
  \hline
 & \multirow{2}{*}{All} & \multicolumn{3}{c}{Age} & &\multicolumn{3}{c}{Emotion}  \\
\cline{3-5}\cline{7-9}
 && Senior & Adult & Child & & Pos & Neg & Neu  \\
\hline
% \textbf{QWEN    } & 1.7           & 0             & 2.5           & 0             && 2             & 0             & 0             \\
% \textbf{Pictor }  & \textbf{98.3} & \textbf{100}  & \textbf{97.5} & \textbf{100}  && \textbf{98}   & \textbf{100}  & \textbf{100}  \\
\textbf{llava7b  }& 19.5          & 15.4          & 25.9          & 0             && 18.4          & 23.5          & 33.3          \\
Pcitor   & \textbf{78.8} & \textbf{84.6} & \textbf{71.6} & \textbf{100}  && \textbf{79.6} & \textbf{76.5} & \textbf{66.7} \\\hline
\textbf{blip}     & 3.4           & 7.7           & 3.7           & 0             && 3.1           & 5.9           & 0             \\
Pictor   & \textbf{96.6} & \textbf{92.3} & \textbf{96.3} & \textbf{100}  && \textbf{96.9} & \textbf{94.1} & \textbf{100}  \\\hline
llava13b & 28.8          & 46.2          & 34.6          & 0             && 24.5          & \textbf{52.9 }& 33.3          \\
Pictor   & 71.2          & 53.9          & 65.4          & 100           && 75.5          & 47.1          & 66.7          \\\hline
gpt4     & 30.5          & 30.8          & 38.3          & 4.2           && 28.6          & 41.2          & 33.3          \\
Pictor            & \textbf{69.5} & \textbf{69.2} & \textbf{61.7} & \textbf{95.8} && \textbf{71.4} & \textbf{58.8} & \textbf{66.7}
\end{tabular}%
}
\caption{This is table}
\label{tab:model_compare}
\end{table}

==> temp.tex <==

% Prompt for dialogue contents consistency
\begin{table*}[]
\centering
\label{tab:consistency}
\begin{tabular}{l}\hline
Prompt for Dialogue Contents Consistency
 \\ \hline
 \small
\texttt{``````$\setminus$}\\

\small\texttt{You are an expert in dialogue quality assessment.} \\
\small\texttt{Below is a two dialogue. First is original one, and second one is system utterance for user} \\
\small\texttt{tailored version.} \\
\small\texttt{Please evaluate the system utterance paraphrased version has the same meaning as the original one.} \\
\small\texttt{This is user image description : \{user\_desc\}} \\
\small\texttt{It is ok to have some difference in wording, that does not change the dialogue process} \\
\small\texttt{significantly.} \\
\small\texttt{If it has same meaning, answer with ``True"; if not, answer with ``False".} \\
\small\texttt{Give only one overall result. Answer in dictionary format to make it easy to parse.} \\
\small\texttt{<Original Dialogue>}\\
\small\texttt{\quad \{org\_dial\}}\\
\small\texttt{<Paraphrased Dialogue>}\\
\small\texttt{\quad \{new\_dial\}}\\
\small\texttt{Evaluation}\\
\small\texttt{Explanation : [explanation], Use : [True or False] $\setminus$}\\


\small
\texttt{""" } \\
\hline

\end{tabular}
\caption{Prompt template for dialogue contents consistency.}
\end{table*}
